An Axiomatic Perspective on the Performance Effects of End-Host Path Selection

In various contexts of networking research, end-host path selection has recently regained momentum as a design principle. While such path selection has the potential to increase performance and security of networks, there is a prominent concern that it could also lead to network instability (i.e., flow-volume oscillation) if paths are selected in a greedy, load-adaptive fashion. However, the extent and the impact vectors of instability caused by path selection are rarely concretized or quantified, which is essential to discuss the merits and drawbacks of end-host path selection. In this work, we investigate the effect of end-host path selection on various metrics of networks both qualitatively and quantitatively. To achieve general and fundamental insights, we leverage the recently introduced axiomatic perspective on congestion control and adapt it to accommodate joint algorithms for path selection and congestion control, i.e., multi-path congestion-control protocols. Using this approach, we identify equilibria of the multi-path congestion-control dynamics and analytically characterize these equilibria with respect to important metrics of interest in networks (the 'axioms') such as efficiency, fairness, and loss avoidance. Moreover, we analyze how these axiomatic ratings for a general network change compared to a scenario without path selection, thereby obtaining an interpretable and quantititative formalization of the performance impact of end-host path-selection. Finally, we show that there is a fundamental trade-off in multi-path congestion-control protocol design between efficiency, stability, and loss avoidance on one side and fairness and responsiveness on the other side.

==> tikzlibraryspline.code.tex <==
%% tikzlibraryspline.code.tex
%% Copyright (C) 2018 Stephen Checkoway
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License version 1.3c.
%
% Version 1.3c of this license is available at
%   http://www.latex-project.org/lppl/lppl-1-3c/
% and is included in the LICENSE file.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Stephen Checkoway.
%
% This work consists of the file tikzlibraryspline.code.tex.

%% Some notes about the implementation.
% This library computes cubic bezier splines through some given points K[0],
% K[1], ..., K[n]. In the case of a closed curve, the user specifies only
% K[0], K[1], ..., K[n-1] and K[n] is taken to be K[0].
%
% A spline (for our purposes) is a piecewise cubic curve consisting of n
% cubic curves connected where segment i starts at point K[i] and ends at
% point K[i+1].
%
% This code and documentation uses the term "knot" to refer to the K[i].
% Traditionally, a knot refers to "time" values, one of the t[0], t[1], ...,
% t[n] values such that S[t[i]] = K[i]. Hopefully, this won't cause too much
% confusion.
%
% The bezier curve control points are calculated by writing the parametric
% equations of each cubic curve and constraining the first and second
% derivatives.
%
% Specifically, we have the n functions
%
%    f_i(t) = (1-t)^3 K[i] + (1-t)^2 t P[i] + (1-t)t^2 Q[i] + t^3 K[i+1]
%
% for i in {0,1,...,n-1} and 0 <= t <= 1. For a closed spline, K[n] = K[0].
%
% For a closed curve, we construct 2n equations in 2n variables by
% requiring differentiating and setting f_{i+1}'(0) = f_i'(1) and
% f_{i+1}''(0) = f_i''(1).
%
% Otherwise, we have 2n-2 equations of that form for the interior knot points.
% By setting f_0''(0) = 0 and f_{n-1}''(1) = 0, we get a total of 2n
% functions.
%
% By some simple algebraic substitution, we can make a system of n equations
% in P[0], P[1], ..., P[n-1]. In the closed case, we have
%
%     P[i-1] + 4P[i] + P[i+1] = 4K[i] + 2K[i+1].
%
% where all indices are taken modulo n. This leads to the linear system AP = R
% where R is the vector of values from the RHS and
%
%    A = [4 1       1
%         1 4 1
%           1 4 1
%               ...
%         1       1 4]
%
% We can solve this linear system in linear time by using the Sherman-Morrison
% formula. In essence, we compute A'P = R, A'z = u where
%
%    A' = [3 1
%          1 4 1
%            1 4 1
%                ...
%                  1 3], and
%     u = [1 0 ... 0 1]^T.
%
% This choice of u is unusual but works well with the fixed point numbers
% we're working with.
%
% Finally, if x[i] and y[i] are the coordinates of P[i], we compute
%
%    fx = (x[0] + x[n-1])/(1 + z[0] + z[n-1]), and
%    fy = (y[0] + y[n-1])/(1 + z[0] + z[n-1]).
%
% and finally update P[i] by setting
%
%    x[i] <- x[i] - fx*z[i]
%    y[i] <- y[i] - fy*z[i].
%
% This gives us the first control point for each segment. From the curve
% equations, we get
%
%    Q[i] = 2K[i+1] - P[i+1]
%
% where again, the indices are taken modulo n.
%
% The situation for the non-closed case is simpler. We have the system of n
% equations in P[0], P[1], ..., P[n-1].
%
%               2P[0]    + P[1]   =  K[0]   + 2K[1]
%      P[i-1] + 4P[i]    + P[i+1] = 2K[i]   + 2K[i+1]  for 0 < i < n-1
%     2P[n-2] + 7P[n-1]           = 8K[n-1] + K[n].
%
% This leads to the linear equation BP = R where elements of R are again the
% RHS of the equations and
%
%    B = [2 1
%         1 4 1
%           1 4 1
%               ...
%                 2 7].
%
% Solving for P gives us the first control point of each segment. The second
% control point Q[i] can be computed via
%
%    Q[i]   = 2K[i+1] - P[i+1] for 0 <= i < n-1
%    Q[n-1] = (K[n] + P[n-1])/2.
%
% That just leaves us with the task of solving these linear systems. Note that
% both A' and B are diagonally dominant tridiagonal matrices. We can solve
% these using the Thomas algorithm.
%
% In general, a tridiagonal matrix has the form
%    [b[0] c[0]
%     a[1] b[1] c[1]
%          a[2] b[2] c[2]
%                       ...
%                         a[n-1] b[n-1]].
% In our case,
%
%    a[i]   = 1 for 0 <= i < n-1
%    a[n-1] = 1 if the spline is closed, otherwise 2
%    b[0]   = 3 if the spline is closed, otherwise 2
%    b[i]   = 4 for 1 <= i < n-1
%    b[n-1] = 3 if the spline is closed, otherwise 7
%    c[i]   = 1 for 0 <= i <= n-1
%
% There are several variants of the algorithm. This performs the following
% steps.
%
% First, the elements below the main diagonal are eliminated by iterating over
% each row i > 0 and replacing it with an appropriate linear combination with
% the previous row. That is, for i=1 up to i=n-1,
%
%    b[i] <- b[i] - a[i]c[i-1]/b[i-1]
%    R[i] <- R[i] - a[i]R[i-1]/b[i-1]
%    u[i] <- u[i] - a[i]u[i-1]/b[i-1] for the closed spline case.
%
% Note that this can be simplified since iterations i=1 through i=n-2
% all have a[i] = 1, b[i] = 4, c[i] = 1, and u[i] = 0.
%
% In fact, the modified b[i] is a function of b[0] (which is either 3 or 2)
% and can be computed via the recurrance b[i] = 4 - 1/b[i]. This converges to
% 2+sqrt(3) regardless of b[0]. For b[0] = 2 or 3, and i > 6, b[i] - b[6] is
% smaller than we can represent. Thus, we can just have a look up table for
% the first 7 values for each of the two starting conditions.
%
% once the lower diagonal has been eliminated, back substitution gives our
% solutions. That is,
%
%    P[n-1] = R[n-1]/b[n-1]
%    z[n-1] = u[n-1]/b[n-1]
%
% and for i=n-2 down to i=0,
%
%    P[i] = (R[i] - c[i]P[i+1])/b[i]
%    z[i] = (u[i] - c[i]z[i+1])/b[i].
%
% Again, we have c[i] = 1 and can look b[i] up in a table.
%
% That's the whole algorithm.
%
% Once we have the control points P[i] and Q[i], we can use pgf to add the
% cublic curve which in pseudo-TikZ notation is:
%
%    .. controls P[i] and Q[i] .. K[i+1]
%
% If nodes are used as knot points, the intersections library is used to
% compute the intersection point between the shape's background path and the
% curve and pgf is used to add just the segment of the curve that's visible.
% TikZ's normal behavior for (A) .. controls (B) and (C) .. (D) when one of
% (A) or (D) is s node is not great, but it's okay. For the spline, it looks
% terrible.

\ProvidesFile{tikzlibraryspline.code.tex}%
  [2018/03/13 v1.0.0 Cubic bezier spline library]
\usepgflibrary{intersections}

\newif\iftikz@spline@closed
\newif\iftikz@spline@usetime
\newcount\tikz@spline@i

\let\tikz@spline@debug=\pgfutil@gobble
\let\tikz@spline@name=\relax

\tikzset{
  spline through/.style={%
    to path={%
      \pgfextra
      \tikz@spline@closedfalse
      \tikz@splinethrough{(\tikztostart)#1(\tikztotarget)}%
      \tikztonodes
    },%
  },
  spline through/.value required,
  closed spline through/.style={%
    to path={%
      \pgfextra
      \tikz@spline@closedtrue
      \let\tikztotarget=\tikztostart
      \tikz@splinethrough{(\tikztostart)#1}%
      \tikztonodes
    }%
  },%
  closed spline through/.value required,
  spline coordinates/.store in=\tikz@spline@name,
  spline coordinates/.default=spline,
  spline debug/.store in=\tikz@spline@debug,
  spline debug/.default=\typeout
}

% Helpers
\def\tikz@spline@save@C#1{%
  \expandafter\edef\csname tikz@spline@C\number#1\endcsname
}

\def\tikz@spline@get@C#1{%
  \csname tikz@spline@C\number#1\endcsname
}

\def\tikz@spline@save@K#1{%
  \expandafter\edef\csname tikz@spline@K\number#1\endcsname
}

\def\tikz@spline@get@K#1{%
  \csname tikz@spline@K\number#1\endcsname
}

% Start the spline construction process.
\def\tikz@splinethrough#1{%
  % Step 1. Parse all of the knots.
  \tikz@spline@i=0
  \tikz@scan@one@point\tikz@spline@knot#1\pgf@stop
}

% Handle a knot by saving the coordinates and the name.
\def\tikz@spline@knot#1{%
  \tikz@make@last@position{#1}%
  \tikz@spline@debug{Parsed point: (\the\tikz@lastx,\the\tikz@lasty) \detokenize{#1}}%
  \tikz@spline@save@K{\tikz@spline@i}{%
    \pgf@x=\the\tikz@lastx
    \pgf@y=\the\tikz@lasty
    \iftikz@shapeborder
      \def\noexpand\tikz@shapeborder@name{\tikz@shapeborder@name}%
    \else
      \let\noexpand\tikz@shapeborder@name\relax
    \fi
  }%
  \advance\tikz@spline@i by1
  \pgfutil@ifnextchar\pgf@stop{%
    \tikz@spline@check@knots
  }{%
    \tikz@scan@one@point\tikz@spline@knot
  }%
}

% Check if we can proceed with the spline contruction.
\def\tikz@spline@check@knots\pgf@stop{%
  % Step 2. Make sure that a closed spline has at least three knots. If the
  % spline is not closed, then we have one fewer segments than knots.
  \let\tikz@next=\tikz@splinethroughA
  \iftikz@spline@closed
    \ifnum\tikz@spline@i<3
      \tikzerror{Closed splines require at least three points}%
      \edef\tikz@next{%
        \noexpand\endpgfextra
        --(\the\tikz@lastx,\the\tikz@lasty)%
      }%
    \fi
  \else
    % If the curve is not closed, there are n-1 segments with n knots
    \advance\tikz@spline@i by-1
  \fi
  % Keep track of how many bezier curve segments we'll be creating.
  \tikz@spline@debug{Creating a spline with \the\tikz@spline@i\space segments}%
  \mathchardef\tikz@spline@segments=\tikz@spline@i
  \tikz@next
}

% Continue the spline construction.
\def\tikz@splinethroughA{%
  % Step 3. Compute the control points P[i].
  \tikz@spline@computeP
  % Step 4. Compute the control points Q[i].
  \tikz@spline@computeQ
  % Step 5. Add the bezier curve segments to the path.
  \tikz@spline@path
  % Step 6. Optionally add coordinates for the control and knot points.
  \ifx\tikz@spline@name\relax\else
    \tikz@spline@i=0
    \tikz@spline@coordinates
    \xdef\tikzsplinesegments{\number\tikz@spline@segments}%
  \fi
  % Done!
  \endpgfextra
}

% Look up the new b (which we're calling bb) values in our table. Read the
% description of the algorithm for how these are computed. For i=n-1, we look
% up n-2 and then compute bb[n-1] = b[n-1] - a[n-1]/bb[n-2].
\def\tikz@spline@lookup@bb#1{%
  \c@pgf@counta=#1\relax
  \advance\c@pgf@counta by1
  \ifnum\c@pgf@counta=\tikz@spline@segments
    % bb[n-1]
    \advance\c@pgf@counta by-2
    \iftikz@spline@closed
      % a/b = bb[n-2]
      \tikz@spline@lookup@closed{\c@pgf@counta}%
      % We want bb[n-1] = (3a - b)/a so set d = 3a - b.
      \c@pgf@countd=\c@pgf@counta
      \multiply\c@pgf@countd by3
      \advance\c@pgf@countd by-\c@pgf@countb
    \else
      % a/b = bb[n-2]
      \tikz@spline@lookup@open{\c@pgf@counta}%
      % We want bb[n-1] = (7a - 2b)/a so set d = 7a - 2b.
      \c@pgf@countd=\c@pgf@counta
      \multiply\c@pgf@countd by7
      \advance\c@pgf@countd by-\c@pgf@countb
      \advance\c@pgf@countd by-\c@pgf@countb
    \fi
    \c@pgf@countb=\c@pgf@counta
    \c@pgf@counta=\c@pgf@countd
  \else
    % bb[i]
    \advance\c@pgf@counta by-1
    \iftikz@spline@closed
      \tikz@spline@lookup@closed{\c@pgf@counta}%
    \else
      \tikz@spline@lookup@open{\c@pgf@counta}%
    \fi
  \fi
}

\def\tikz@spline@lookup@closed#1{%
  % First, assign to a and then assign to b
  \afterassignment\c@pgf@countb
  \c@pgf@counta=\ifcase#1%
        3 1%
    \or 11 3%
    \or 41 11%
    \or 153 41%
    \or 571 153%
    \or 2131 571%
    \else 7953 2131%
  \fi
  \relax % We need a single token to end the second expansion.
}

\def\tikz@spline@lookup@open#1{%
  \afterassignment\c@pgf@countb
  \c@pgf@counta=\ifcase#1%
        2 1%
    \or 7 2%
    \or 26 7%
    \or 97 26%
    \or 362 97%
    \or 1351 362%
    \else 5042 1351%
  \fi
  \relax
}

% Step 3. Compute the control points P[i] by solving AP = R.
\def\tikz@spline@computeP{%
  % Perform the first step of the forward sweep of solving the tridiagonal (or
  % cyclic) matrix equation.
  \tikz@spline@get@K{0}%
  \iftikz@spline@closed
    % R[0] = 4K[0] + 2K[1]
    \pgf@xa=4\pgf@x
    \pgf@ya=4\pgf@y
  \else
    % R[0] = K[0] + 2*K[1]
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
  \fi
  \tikz@spline@get@K{1}%
  \advance\pgf@xa by2\pgf@x
  \advance\pgf@ya by2\pgf@y
  % x[0] = rx[0]
  % y[0] = ry[0]
  % z[0] = 1
  \pgf@xc=1pt
  \tikz@spline@save@C{0}{%
    \pgf@xa=\the\pgf@xa
    \pgf@ya=\the\pgf@ya
    \pgf@xc=\the\pgf@xc
  }%
  \tikz@spline@lookup@bb{0}%
  \tikz@spline@debug{%
    0: bb=\the\c@pgf@counta/\the\c@pgf@countb,
    x=\the\pgf@xa,
    y=\the\pgf@ya,
    z=\the\pgf@xc%
  }%
  \tikz@spline@i=1
  \c@pgf@countc=2
  \tikz@spline@computePA
}

% Step 3a. Handle all forward sweeping steps up to segments-2.
\def\tikz@spline@computePA{%
  % At this point,
  % \pgf@x/\pgf@y = K[i]
  % \pgf@xa/\pgf@ya = P[i-1]
  % \pgf@xc = z[i-1]
  % \c@pgf@counta/\c@pgf@countb = bb[i-1]
  %
  % R[i] = 4*K[i] + 2*K[i+1]
  \pgf@xb=4\pgf@x
  \pgf@yb=4\pgf@y
  \tikz@spline@get@K{\c@pgf@countc}%
  \advance\pgf@xb by2\pgf@x
  \advance\pgf@yb by2\pgf@y
  % P[i] = R[i] - P[i-1]/bb[i-1]
  % z[i] = 0 - z[i-1]/bb[i-1]
  \pgf@xa=\dimexpr\pgf@xb-\pgf@xa*\c@pgf@countb/\c@pgf@counta\relax
  \pgf@ya=\dimexpr\pgf@yb-\pgf@ya*\c@pgf@countb/\c@pgf@counta\relax
  \pgf@xc=\dimexpr-\pgf@xc*\c@pgf@countb/\c@pgf@counta\relax
  \tikz@spline@save@C{\tikz@spline@i}{%
    \pgf@xa=\the\pgf@xa
    \pgf@ya=\the\pgf@ya
    \pgf@xc=\the\pgf@xc
  }%
  \tikz@spline@lookup@bb{\tikz@spline@i}%
  \tikz@spline@debug{%
    \the\tikz@spline@i:
    bb=\the\c@pgf@counta/\the\c@pgf@countb,
    x=\the\pgf@xa,
    y=\the\pgf@ya,
    z=\the\pgf@xc%
  }%
  \advance\tikz@spline@i by1
  \advance\c@pgf@countc by1
  \ifnum\c@pgf@countc=\tikz@spline@segments
    \expandafter\tikz@spline@computePB
  \else
    \expandafter\tikz@spline@computePA
  \fi
}


% Step 3b. Handle the last iteration of the forward sweep and the first
% iteration of the backwards substitution.
\def\tikz@spline@computePB{%
  % At this point,
  % \pgf@x/\pgf@y = K[n-1]
  % \pgf@xa/\pgf@ya = P[n-2]
  % \pgf@xc = z[n-2]
  % \c@pgf@counta/\c@pgf@countb = bb[n-2]
  \iftikz@spline@closed
    \pgf@xb=4\pgf@x
    \pgf@yb=4\pgf@y
    \tikz@spline@get@K{0}%
    \advance\pgf@xb by2\pgf@x
    \advance\pgf@yb by2\pgf@y
    % P[n-1] = R[n-1] - P[n-2]/bb[n-2]
    % z[n-1] = 1 - z[n-2]/bb[n-2]
  \else
    % R[n-1] = 8K[n-1] + K[n]
    \pgf@xb=8\pgf@x
    \pgf@yb=8\pgf@y
    \tikz@spline@get@K{\c@pgf@countc}%
    \advance\pgf@xb by\pgf@x
    \advance\pgf@yb by\pgf@y
    % P[n-1] = R[n-1] - 2P[n-2]/bb[n-2]
    \advance\c@pgf@countb by\c@pgf@countb
  \fi
  \pgf@xa=\dimexpr\pgf@xb-\pgf@xa*\c@pgf@countb/\c@pgf@counta\relax
  \pgf@ya=\dimexpr\pgf@yb-\pgf@ya*\c@pgf@countb/\c@pgf@counta\relax
  \pgf@xc=\dimexpr1pt-\pgf@xc*\c@pgf@countb/\c@pgf@counta\relax
  % No need to save these since we're going to use them immediately.
  %
  % P[n-1] = P[n-1]/bb[n-1]
  % z[n-1] = z[n-1]/bb[n-1]
  \tikz@spline@lookup@bb{\tikz@spline@i}%
  \tikz@spline@debug{%
    \the\tikz@spline@i:
    bb=\the\c@pgf@counta/\the\c@pgf@countb,
    x=\the\pgf@xa,
    y=\the\pgf@ya,
    z=\the\pgf@xc%
  }%
  % Store P[n-1] in \pgf@xb/\pgf@yb and z[n-1] in \pgf@yc
  \pgf@xb=\dimexpr\pgf@xa*\c@pgf@countb/\c@pgf@counta\relax
  \pgf@yb=\dimexpr\pgf@ya*\c@pgf@countb/\c@pgf@counta\relax
  \pgf@yc=\dimexpr\pgf@xc*\c@pgf@countb/\c@pgf@counta\relax
  \tikz@spline@save@C{\tikz@spline@i}{%
    \pgf@xa=\the\pgf@xb
    \pgf@ya=\the\pgf@yb
    \pgf@xc=\the\pgf@yc
  }%
  \tikz@spline@debug{%
    \the\tikz@spline@i:
    bb=\the\c@pgf@counta/\the\c@pgf@countb,
    x=\the\pgf@xb,
    y=\the\pgf@yb,
    z=\the\pgf@yc%
  }%
  \def\tikz@next{\tikz@spline@computePC}%
  \tikz@spline@computePC
}

% Step 3c. Handle all of the rest of the backwards substitutions.
\def\tikz@spline@computePC{%
  \advance\tikz@spline@i by-1
  % At this point,
  % \pgf@xb/\pgf@yb = P[i+1]
  % \pgf@yc = z[i+1]
  %
  % P[i] = (P[i] - P[i+1])/bb[i]
  % z[i] = (z[i] - z[i+1])/bb[i]
  \tikz@spline@lookup@bb{\tikz@spline@i}%
  \tikz@spline@get@C{\tikz@spline@i}%
  \pgf@xb=\dimexpr(\pgf@xa-\pgf@xb)*\c@pgf@countb/\c@pgf@counta\relax
  \pgf@yb=\dimexpr(\pgf@ya-\pgf@yb)*\c@pgf@countb/\c@pgf@counta\relax
  \pgf@yc=\dimexpr(\pgf@xc-\pgf@yc)*\c@pgf@countb/\c@pgf@counta\relax
  \tikz@spline@save@C{\tikz@spline@i}{%
    \pgf@xa=\the\pgf@xb
    \pgf@ya=\the\pgf@yb
    \pgf@xc=\the\pgf@yc
  }%
  \tikz@spline@debug{%
    \the\tikz@spline@i:
    bb=\the\c@pgf@counta/\the\c@pgf@countb,
    x=\the\pgf@xb,
    y=\the\pgf@yb,
    z=\the\pgf@yc%
  }%
  \ifnum\tikz@spline@i=0
    \tikz@spline@i=\tikz@spline@segments
    \iftikz@spline@closed
      % Goto step 3d.
      \def\tikz@next{\tikz@spline@computePD}%
    \else
      % Done with step 3.
      \let\tikz@next=\relax
    \fi
  \fi
  \tikz@next
}

% Step 3d. For a closed spline, compute the appropriate factor and then
% multiply P[i] by the factor for each i.
\def\tikz@spline@computePD{%
  % d = 1 + z[0] + z[n-1]
  % fx = (x[0] + x[n-1])/d
  % fy = (y[0] + y[n-1])/d
  \advance\tikz@spline@i by-1
  \tikz@spline@get@C{\tikz@spline@i}%
  \pgf@xb=\pgf@xa
  \pgf@yb=\pgf@ya
  \pgf@yc=\pgf@xc
  \tikz@spline@get@C{0}%
  \advance\pgf@xc by\pgf@yc
  \advance\pgf@xc by1pt
  \advance\pgf@xa by\pgf@xb
  \advance\pgf@ya by\pgf@yb
  \c@pgf@counta=\pgf@xc
  \pgf@xc=\dimexpr\pgf@xa*65536/\c@pgf@counta\relax
  \pgf@yc=\dimexpr\pgf@ya*65536/\c@pgf@counta\relax
  \edef\tikz@spline@fx{\pgf@sys@tonumber\pgf@xc}%
  \edef\tikz@spline@fy{\pgf@sys@tonumber\pgf@yc}%
  \tikz@spline@i=\tikz@spline@segments
  \tikz@spline@computePE
}

% Step 3e. For a closed spline only. Iterate through each segment and
% modify P appropriately.
\def\tikz@spline@computePE{%
  \advance\tikz@spline@i by-1
  \tikz@spline@get@C{\tikz@spline@i}%
  % Px[i] = Px[i] - fx*z[i]
  % Py[i] = Py[i] - fy*z[i]
  \advance\pgf@xa by-\tikz@spline@fx\pgf@xc
  \advance\pgf@ya by-\tikz@spline@fy\pgf@xc
  \tikz@spline@save@C{\tikz@spline@i}{%
    \pgf@xa=\the\pgf@xa
    \pgf@ya=\the\pgf@ya
  }%
  \ifnum\tikz@spline@i=0
    \let\tikz@spline@fx=\@undefined
    \let\tikz@spline@fy=\@undefined
  \else
    \expandafter\tikz@spline@computePE
  \fi
}

% Step 4. Compute control points Q[i].
\def\tikz@spline@computeQ{%
  \tikz@spline@i=\tikz@spline@segments
  \iftikz@spline@closed
    % Q[n-1] = 2K[0] - P[0]
    \advance\tikz@spline@i by-1
    \tikz@spline@get@K{0}%
    \tikz@spline@get@C{0}%
    \pgf@xb=2\pgf@x
    \pgf@yb=2\pgf@y
    \advance\pgf@xb by-\pgf@xa
    \advance\pgf@yb by-\pgf@ya
    \tikz@spline@get@C{\tikz@spline@i}%
  \else
    % Q[n-1] = (K[n] + P[n-1])/2
    \tikz@spline@get@K{\tikz@spline@i}%
    \advance\tikz@spline@i by-1
    \tikz@spline@get@C{\tikz@spline@i}%
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \advance\pgf@xb by\pgf@xa
    \advance\pgf@yb by\pgf@ya
    \divide\pgf@xb by2
    \divide\pgf@yb by2
  \fi
  \tikz@spline@save@C{\tikz@spline@i}{%
    \pgf@xa=\the\pgf@xa
    \pgf@ya=\the\pgf@ya
    \pgf@xb=\the\pgf@xb
    \pgf@yb=\the\pgf@yb
  }%
  \tikz@spline@debug{%
    P[\the\tikz@spline@i]=(\the\pgf@xa,\the\pgf@ya)
    Q[\the\tikz@spline@i]=(\the\pgf@xb,\the\pgf@yb)%
  }%
  \tikz@spline@computeQA
}

% Step 4a. Compute the rest of the Q[i] = 2K[i+1] - P[i+1]
\def\tikz@spline@computeQA{%
  \tikz@spline@get@K{\tikz@spline@i}%
  \tikz@spline@get@C{\tikz@spline@i}%
  \pgf@xb=2\pgf@x
  \pgf@yb=2\pgf@y
  \advance\pgf@xb by-\pgf@xa
  \advance\pgf@yb by-\pgf@ya
  \advance\tikz@spline@i by-1
  \tikz@spline@get@C{\tikz@spline@i}%
  \tikz@spline@save@C{\tikz@spline@i}{%
    \pgf@xa=\the\pgf@xa
    \pgf@ya=\the\pgf@ya
    \pgf@xb=\the\pgf@xb
    \pgf@yb=\the\pgf@yb
  }%
  \tikz@spline@debug{%
    P[\the\tikz@spline@i]=(\the\pgf@xa,\the\pgf@ya)
    Q[\the\tikz@spline@i]=(\the\pgf@xb,\the\pgf@yb)%
  }%
  \ifnum\tikz@spline@i=0\else
    \expandafter\tikz@spline@computeQA
  \fi
}

% Step 5. Add the bezier curve segments to the path.
\def\tikz@spline@path{%
  \tikz@spline@i=0
  \tikz@spline@pathA
  \let\tikz@timer=\tikz@spline@timer
}

\def\tikz@spline@select@segment#1{%
  \c@pgf@counta=#1\relax
  \tikz@spline@get@K{\c@pgf@counta}%
  \tikz@spline@get@C{\c@pgf@counta}%
  \edef\tikz@spline@zeroth{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \let\tikz@spline@startname=\tikz@shapeborder@name
  \edef\tikz@spline@first{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \edef\tikz@spline@second{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
  \advance\c@pgf@counta by1
  \ifnum\c@pgf@counta=\tikz@spline@segments
    \iftikz@spline@closed
      % The end knot is the start knot.
      \c@pgf@counta=0
    \fi
  \fi
  \tikz@spline@get@K{\c@pgf@counta}%
  \edef\tikz@spline@third{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \let\tikz@spline@endname=\tikz@shapeborder@name
}

% Step 5a.
\def\tikz@spline@pathA{%
  \tikz@spline@select@segment{\tikz@spline@i}%
  % If the start or end coordinates are shapes, calculate the intersection
  % times.
  \tikz@spline@usetimefalse
  \def\tikz@spline@timea{0}%
  \def\tikz@spline@timeb{1}%
  \ifx\tikz@spline@startname\relax\else
    \pgfutil@ifundefined{pgf@sh@bg@\csname pgf@sh@ns@\tikz@spline@startname\endcsname}{}{%
      % Defined.
      \tikz@spline@border@time{\tikz@spline@startname}{\tikz@spline@timea}{1}%
      \tikz@spline@usetimetrue
    }%
  \fi
  % Check for an end shape
  \ifx\tikz@spline@endname\relax\else
    \pgfutil@ifundefined{pgf@sh@bg@\csname pgf@sh@ns@\tikz@spline@endname\endcsname}{}{%
      \tikz@spline@border@time{\tikz@spline@endname}{\tikz@spline@timeb}{\pgfintersectionsolutions}%
      \tikz@spline@usetimetrue
    }%
  \fi
  % If either end point was a shape, use \pgfpathcurvebetweentime to draw part
  % of the curve.
  \iftikz@spline@usetime
    \pgfpathcurvebetweentime{\tikz@spline@timea}{\tikz@spline@timeb}%
      {\tikz@spline@zeroth}{\tikz@spline@first}{\tikz@spline@second}{\tikz@spline@third}%
  \else
    \pgfpathcurveto{\tikz@spline@first}{\tikz@spline@second}{\tikz@spline@third}%
  \fi
  \ifnum\tikz@spline@i=0
    % Save the start time for the timer.
    \let\tikz@spline@starttime=\tikz@spline@timea
  \fi
  \advance\tikz@spline@i by1
  \ifnum\tikz@spline@i=\tikz@spline@segments
    \ifdim\tikz@spline@timeb pt<1pt
      % \pgfpointcurveattime puts points on the tangent in xa/ya and xb/yb.
      % XXX: This was computed from the intersection before, we could reuse
      % it.
      \pgfpointcurveattime{\tikz@spline@timeb}{\tikz@spline@zeroth}%
        {\tikz@spline@first}{\tikz@spline@second}{\tikz@spline@third}%
      \edef\tikz@tangent{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@yb}}%
      \tikz@make@last@position{}% \pgf@x/\pgf@y already contain the position.
    \else
      % The end point of the curve is the last position and the second control
      % point is on the tangent.
      \let\tikz@tangent=\tikz@spline@second
      \tikz@make@last@position{\tikz@spline@third}%
    \fi
    \let\tikz@spline@endtime=\tikz@spline@timeb
  \else
    \expandafter\tikz@spline@pathA
  \fi
}

% \tikz@spline@border@time{node}{\time}{which solution}
\def\tikz@spline@border@time#1#2#3{
  \begingroup
  \pgfintersectionofpaths{%
    \pgfpathmoveto{\tikz@spline@zeroth}%
    \pgfpathcurveto{\tikz@spline@first}{\tikz@spline@second}{\tikz@spline@third}%
  }{%
    % Install special macros (cargo-cult programming, I don't know what these
    % are or why they're important)
    \csname pgf@sh@ma@#1\endcsname
    % Install special coordinates (things like \radius and \centerpoint)
    \csname pgf@sh@np@#1\endcsname
    % Set the transform
    \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
    % Create the background path
    \csname pgf@sh@bg@\csname pgf@sh@ns@#1\endcsname\endcsname
  }
  \ifnum\pgfintersectionsolutions=0
    \tikz@spline@debug{Unable to find an intersection between `#1' and the spline}
    \pgf@process{%
      \ifnum#3=0
        \tikz@spline@zeroth
      \else
        \tikz@spline@third
      \fi
    }%
  \else
    \pgfintersectiongetsolutiontimes{#3}{#2}{\tikz@spline@dummy}%
  \fi
  \edef\tikz@marshal{\endgroup\def\noexpand#2{#2}}%
  \tikz@marshal
}

% Transform \tikz@time to a point along the spline. If the start or end are
% shapes, then times 0 and 1 correspond to intersection points with the
% border.
\def\tikz@spline@timer{%
  % Compute the segment number in \tikz@spline@i
  \pgf@xa=\tikz@time \tikz@spline@segments
  \tikz@spline@i=\pgf@xa
  % Compute the fractional part in \pgf@xa
  \ifnum\tikz@spline@i=\tikz@spline@segments
    \advance\tikz@spline@i by-1
    \pgf@xa=1pt
  \else
    \pgf@xa=\tikz@time pt
    \pgf@xa=\tikz@spline@segments \pgf@xa
    \advance\pgf@xa by -\tikz@spline@i pt
  \fi
  % Determine the start and end of the segments
  \ifnum\tikz@spline@i=0
    \pgf@xb=\tikz@spline@starttime pt
  \else
    \pgf@xb=0pt
  \fi
  \c@pgf@countc=\tikz@spline@i
  \advance\c@pgf@countc by1
  \ifnum\c@pgf@countc=\tikz@spline@segments
    \pgf@yb=\tikz@spline@endtime pt
  \else
    \pgf@yb=1pt
  \fi
  % t' = (t - i/n)(yb - xb)/(1/n) = (t*n - i)(yb - xb) + xb
  % Put the scaling factor in \pgf@yb
  \advance\pgf@yb by-\pgf@xb
  % Compute scaled and shifted time
  \pgf@xa=\pgf@sys@tonumber{\pgf@yb}\pgf@xa
  \advance\pgf@xa by\pgf@xb
  \edef\tikz@spline@time{\pgf@sys@tonumber{\pgf@xa}}
  % Get the appropriate control points for the segment
  \tikz@spline@select@segment{\tikz@spline@i}%
  \tikz@spline@debug{%
    \string\tikz@time=\tikz@time\space -> \the\tikz@spline@i.\tikz@spline@time
  }%
  \pgftransformcurveattime{\tikz@spline@time}{\tikz@spline@zeroth}{\tikz@spline@first}{\tikz@spline@second}{\tikz@spline@third}%
}

\def\tikz@spline@coordinates{%
  \tikz@spline@get@K{\tikz@spline@i}%
  \tikz@spline@get@C{\tikz@spline@i}%
  \advance\tikz@spline@i by1
  \def\tikz@temp##1{\tikz@spline@name\space ##1-\the\tikz@spline@i}%
  \edef\tikz@marshal{%
    node[shape=coordinate](\tikz@temp{K})at(\the\pgf@x,\the\pgf@y){}%
    node[shape=coordinate](\tikz@temp{P})at(\the\pgf@xa,\the\pgf@ya){}%
    node[shape=coordinate](\tikz@temp{Q})at(\the\pgf@xb,\the\pgf@yb){}%
  }%
  \expandafter\endpgfextra\tikz@marshal
  \pgfextra
  \ifnum\tikz@spline@i=\tikz@spline@segments
    \iftikz@spline@closed
      \tikz@spline@get@K{0}%
    \else
      \tikz@spline@get@K{\tikz@spline@i}%
    \fi
    \advance\tikz@spline@i by1
    \edef\tikz@marshal{%
      node[shape=coordinate](\tikz@temp{K})at(\the\pgf@x,\the\pgf@y){}%
    }%
    \expandafter\endpgfextra\tikz@marshal
    \pgfextra
  \else
    \expandafter\tikz@spline@coordinates
  \fi
}
\endinput
% vim: set sw=2 sts=2 ts=8 et nospell:

